Empowering In-Browser Deep Learning Inference on Edge Devices with Just-in-Time Kernel Optimizations

Web is increasingly becoming the primary platform to deliver AI services onto edge devices, making in-browser deep learning (DL) inference more prominent. Nevertheless, the heterogeneity of edge devices, combined with the underdeveloped state of Web hardware acceleration practices, hinders current in-browser inference from achieving its full performance potential on target devices. To address this issue, this paper presents the pioneering inbrowser inference system, nnJIT, which enables just-in-time (JIT) auto-generation of optimized computing kernels for edge devices. nnJIT is built upon two novel techniques that significantly reduce kernel search and compilation overhead while improving performance firmly: Tensor-Web Compiling Co-Design lowers compiling costs by around 100X through eliminating redundant and ineffective compiling passes; Web-Specific Lite Kernel Optimization Space reduces kernel tuning costs by focusing on Web programming requirements and efficient device resource utilization, pruning the optimization space from millions to only dozens. nnJIT is evaluated for modern models, e.g., BART, T5, and Llama 2, on a range of edge devices including laptops and smartphones using different browsers and hardware from ARM, Intel, AMD and Nvidia. The results show that nnJIT can achieve up to 8.2X faster within 30 seconds compared to the existing baselines.

==> design_high_performance_kernel_generation.tex <==
\section{High-Performance Kernel Generation}

The goal of browser-features- and hardware-capability-aware microbenchmark is to online find the optimal-performance schedule for a in-browser kernel on a specific device. Two principles should be considered into the design of browser-features-aware microbenchmark. First, the kernel schedule should be aware of browser backend features. Second, the kernel schedule configures could be scaled according to the hardware capability (the size of L1 cache, registers, etc.).

\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/tvm_generator_vs_browser_microbenchmark.pdf}
  \caption{The high-level workflow of TVM and our browser-features- and hardware-capability-aware microbenchmark.\ting{update}}
  \Description{}
  \label{F.tvm_generator_vs_browser_microbenchmark}
\end{figure}


There are two challenges for the design of microbenchmark: 1) the browser backend features for kernel schedule searching are not clear; 2) how to online find the optimal kernel schedule by taking the advantages of browser backend features. To address the two challenges, we first demystify the features of two browser backends on kernel schedules. Then, we design an online microbenchmark which can significantly reduce the search space and find the optimal kernel schedule with few steps.


\subsection{WebAssembly feastures demystification}



To understand the features of WebAssembly on kernel schedules, we measure the latency of a MatMul kernel with various schedule primitives on three CPU devices. Our key findings are as follows:


\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/wasm_schedule_tile_size_and_kernel_latency.pdf}
  \caption{The MatMul kernel latency under various (inner+outer) tile sizes on three CPU devices. The input size is [M,K,N]=[640,768,3072]. We enable vectorization and unrolling.}
  \Description{}
  \label{F.wasm_schedule_tile_size_and_kernel_latency}
\end{figure}

\textbf{Non-uniform tile sizes} Xxx.

\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/wasm_schedule_cache_read_write_and_kernel_latency.pdf}
  \caption{The MatMul kernel latency under various cache read (Cr) and cache write (Cw) configures on three CPU devices. The input size is [M,K,N]=[640,768,3072]. We enable vectorization and unrolling.}
  \Description{}
  \label{F.wasm_schedule_cache_read_write_and_kernel_latency}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/wasm_schedule_vectorize_unroll_and_kernel_latency.pdf}
  \caption{The MatMul kernel latency under various vectorization and unrolling configures on three CPU devices. The input size is [M,K,N]=[640,768,3072].}
  \Description{}
  \label{F.wasm_schedule_vectorize_unroll_and_kernel_latency}
\end{figure}

\textbf{Uniform cache read/write, vectorization and unrolling} Xxx.






\begin{algorithm}[t]
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
  \Input{Kernel Expression $ke$, local CPU capability $cpuCap$}
  \Output{Optimal kernel WebAssembly binary $optKernelWasmBin$}
  $ts0$, $ts1$ $\leftarrow$ $initTileSize$\;
  $minCost$ $\leftarrow$ $curCost$\;
  $optKernelWasmBin$ $\leftarrow$ $null$\;
  \While{$ts0, ts1$ < $maxTileSize$}{
    $inTile0$, $inTile1$, $outTile$ $\leftarrow$ $ke.Tile(ts0, ts1)$\;
    $ke.Vectorize(inTile0.lastDim, 128)$\;
    $ke.Unroll(inTile0.allDims)$\;
    \If{$EstimateCpuOccupancy(ke, cpuCap) \in [minOccupancy, maxOccupancy]$}{
    $kernelWasmBin$ $\leftarrow$ $Compile(ke)$\;
      $cost$ $\leftarrow$ $Execute(kernelWasmBin)$\;
      \If{$cost$ < $minCost$}{
        $optKernelWasmBin$ $\leftarrow$ $kernelWasmBin$\;
        $minCost$ $\leftarrow$ $cost$\;
      }
    }
    $ts0, ts1$ $\leftarrow$ $Enlarge(ts0, ts1)$\;
  }
\caption{WebAssembly Microbenchmark}
\label{A.wasm_microbenchmark}
\end{algorithm}

\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/microbenchmark_generation_time_and_kernel_performance.pdf}
  \caption{The generation time and MatMul kernel performance of our microbenchmark and TVM on AMD 5800H CPU.}
  \Description{}
  \label{F.microbenchmark_generation_time_and_kernel_performance}
\end{figure}


\subsection{WebGPU feastures demystification}


Similar to WebAssembly Backend, we demysitify the features of WebGPU backend based on the measurement of MatMul kernels on two GPU devices. The key findings are as follow:

\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/webgpu_schedule_tile_size_and_kernel_latency.pdf}
  \caption{The MatMul kernel latency under various (inner+outer) tile sizes on two GPU devices. The input size is [M,K,N]=[640,768,3072].}
  \Description{}
  \label{F.webgpu_schedule_tile_size_and_kernel_latency}
\end{figure}

\textbf{Non-uniform tile sizes} Xxx.

\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/webgpu_schedule_cache_read_write_and_kernel_latency.pdf}
  \caption{The MatMul kernel latency under various cache read (Cr) and cache write (Cw) configures on two GPU devices. The input size is [M,K,N]=[640,768,3072].}
  \Description{}
  \label{F.webgpu_schedule_cache_read_write_and_kernel_latency}
\end{figure}

\textbf{Non-uniform cache read and vectorization} Xxx.

\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/webgpu_schedule_vectorize_unroll_and_kernel_latency.pdf}
  \caption{The MatMul kernel latency under various vectorization and unrolling configures on three CPU devices. The input size is [M,K,N]=[640,768,3072].}
  \Description{}
  \label{F.webgpu_schedule_vectorize_unroll_and_kernel_latency}
\end{figure}

\textbf{Uniform cache write and unrolling} Xxx.









\begin{algorithm}[t]
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
  \Input{Kernel Expression $ke$, local GPU capability $gpuCap$}
  \Output{Optimal kernel WebGPU source code $optKernelCode$}
  $ts0$, $ts1$ $\leftarrow$ $initTileSize$\;
  $minCost$ $\leftarrow$ $curCost$\;
  $optKernelCode$ $\leftarrow$ $null$\;
  \While{$ts0, ts1$ < $maxTileSize$}{
    $inTile0$, $inTile1$, $outTile$ $\leftarrow$ $ke.Tile(ts0, ts1)$\;
    $ke.BindThread(inTile1)$\; $ke.BindBlock(outTile)$\;
    \lIf{$gpuCap.sharedMemoryLevel$ = $L1Cache$}{$ke.SetScope(outTile, "shared")$}
    \lElse{$ke.SetScope(outTile, "global")$}
    \lIf{$gpuCap.isSimd$}{$ke.Vectorize(inTile0.lastDim, 128)$}
    \For{$doUnroll \in [True, False]$}{
      \lIf{$doUnroll$}{$ke.Unroll(inTile0.allDims)$}
      \If{$IsRegisterBound(ke, gpuCap)$ and $EstimateGpuOccupancy(ke, gpuCap) \in [minOccupancy, maxOccupancy]$}{
        $kernelCode$ $\leftarrow$ $CodeGen(ke)$\;
        $cost$ $\leftarrow$ $CompileAndExecute(kernelCode)$\;
        \If{$cost$ < $minCost$}{
          $optKernelCode$ $\leftarrow$ $kernelCode$\;
          $minCost$ $\leftarrow$ $cost$\;
        }
      }
    }
    $ts0, ts1$ $\leftarrow$ $Enlarge(ts0, ts1)$\;
  }
\caption{WebGPU Microbenchmark}
\label{A.webgpu_microbenchmark}
\end{algorithm}


\subsection{Browser-features- and hardware-capability-aware microbenchmark}


==> design_online_kernel_generator.tex <==
\section{Online Kernel Compiler}

\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/tvm_llvm_compiler_vs_wasm_compiler.pdf}
  \caption{The high-level workflow of TVM kernel compilation and our online kernel compiler.\ting{update the graph}}
  \Description{}
  \label{F.tvm_llvm_compiler_vs_wasm_compiler}
\end{figure}

The goal of our online kernel compiler is to compile the optimal kernel schedule to executable binary code. We consider two principles for the online kernel compiler. First, we should directly map kernel schedule to WASM IR without any internal process. Second, we should optimize the mapped WASM IR to avoid redundant memory access. Since the kernel compilation of WebGPU backend does not meet heavy cost issue, we only design the online kernel compiler for WebAssmbly backend.

The high-level workflow of our online kernel compiler is illustrated in Fig. \ref{F.tvm_llvm_compiler_vs_wasm_compiler} (b). Different from TVM kernel compilation, our kernel compiler 1) directly maps TVM IR to WASM IR, 2) leverages simplified IR optimization, and 3) directly generates WASM binary without depending on the heavy compilation toolchains.

\begin{algorithm}[t]
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
  \Input{Kernel IR $kIR$}
  \Output{WebAssembly IR $wasmIR$}
  \SetKwProg{Fn}{Func}{:}{}
  \SetKwFunction{FVisitStmt}{VisitStmt}
  \SetKwFunction{FVisitFunction}{VisitFunction}
  \Fn{\FVisitStmt(node)}{
    \If{$node.type == AddNode$}{
      \lIf{$node.dataType == Int$}{$wasmIR.makeBinary(AddInt32, node.a, node.b)$}
      \lElse{$wasmIR.makeBinary(AddFloat32, node.a, node.b)$}
    }
    \If{$node.type == ...$}{
      ...\;
    }
  }
  \Fn{\FVisitFunction(func)}{
    $wasmIR.makeFunction(func.name, func.params)$\;
    $VisitStmt(func.body)$\;
  }
  $wasmIR$ $\leftarrow$ $InitWasmIR()$\;
  $VisitFunction(kIR.function)$\;
\caption{Direct kernel-to-WASM IR mapping}
\label{A.direct_kernel_to_wasm_ir_mapping}
\end{algorithm}

\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/tvm_ir_map_to_wasm_ir.pdf}
  \caption{A simple example of kernel IR mapping to WebAssembly IR.}
  \Description{}
  \label{F.tvm_ir_map_to_wasm_ir}
\end{figure}

\textbf{Direct kernel-to-WASM IR mapping} Algorithm \ref{A.direct_kernel_to_wasm_ir_mapping} shows the process of direct kernel-to-WASM IR mapping. Xxx. A simple example of kernel-to-WASM IR mapping is illustrated in Fig. \ref{F.tvm_ir_map_to_wasm_ir}.

\begin{algorithm}[t]
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
  \Input{WebAssembly IR $wasmIR$}
  \Output{Optimized WebAssembly IR $optWasmIR$}
  \SetKwProg{Fn}{Func}{:}{}
  \SetKwFunction{FBufferLoadAndStoreRecution}{BufferLoadAndStoreRecution}
  \SetKwFunction{FOffsetConstantization}{OffsetConstantization}
  \SetKwFunction{FInstructionsCombination}{InstructionsCombination}
  \Fn{\FBufferLoadAndStoreRecution(wasmIR)}{
  
  }
  \Fn{\FOffsetConstantization(wasmIR)}{
  
  }
  \Fn{\FInstructionsCombination(wasmIR)}{
  
  }
  $BufferLoadAndStoreRecution(wasmIR)$\;
  $OffsetConstantization(wasmIR)$\;
  $InstructionsCombination(wasmIR)$\;
  $optWasmIR$ $\leftarrow$ $wasmIR$\;
\caption{Light-weight WASM IR optimization}
\label{A.light_weight_wasm_ir_optimization}
\end{algorithm}

\textbf{Simplified WASM IR optimization} Our simplified WASM IR optimization is shown in Algorithm \ref{A.light_weight_wasm_ir_optimization}. The optimization only includes three passes: 1) buffer storing/loading reduction, 2) offset constantization and 3) instructions combination.

Fig. \ref{} shows an example of WASM IR before and after the WASM IR optimization.


==> discussion.tex <==
\section{Discussion}

\textbf{Comparison with cloud-based/5G edge-based solution.} \update{In-browser on-device inference reduces cloud operation costs and provides improved privacy. For example, as stated in \cite{zerocogs}, serving millions of users for a DNN service on the cloud can cost a significant amount of money. On-device inference has the potential to achieve zero cost. Additionally, as stated in \cite{cloudcyberattacks}, there is always a risk of data breaches when information travels over the internet. Given these realities, even though network latency may be less noticeable, on-device inference will still be in high demand.}

\textbf{Potential kernel optimization for memory.} \update{We could include the memory access or memory usage constraints in the heuristics of web-specific lite space. For example, we can search for the least memory access kernels to reduce memory accesses, and constrain $L1_{block}$ in Table \ref{T.specific_paramter} to reduce the usage of shared memory for WebGPU.}

